Graph Neural Network Training Systems: A Performance Comparison of Full-Graph and Mini-Batch

Graph Neural Networks (GNNs) have gained significant attention in recent years due to their ability to learn representations of graph-structured data. Two common methods for training GNNs are mini-batch training and full-graph training. Since these two methods require different training pipelines and systems optimizations, two separate classes of GNN training systems emerged, each tailored for one method. Works that introduce systems belonging to a particular category predominantly compare them with other systems within the same category, offering limited or no comparison with systems from the other category. Some prior work also justifies its focus on one specific training method by arguing that it achieves higher accuracy than the alternative. The literature, however, has incomplete and contradictory evidence in this regard. In this paper, we provide a comprehensive empirical comparison of representative full-graph and mini-batch GNN training systems. We find that the mini-batch training systems consistently converge faster than the full-graph training ones across multiple datasets, GNN models, and system configurations. We also find that mini-batch training techniques converge to similar to or often higher accuracy values than full-graph training ones, showing that mini-batch sampling is not necessarily detrimental to accuracy. Our work highlights the importance of comparing systems across different classes, using time-to-accuracy rather than epoch time for performance comparison, and selecting appropriate hyperparameters for each training method separately.

==> ref.tex <==
@inproceedings{pinsage,
  title={Graph convolutional neural networks for web-scale recommender systems},
  author={Ying, Rex and He, Ruining and Chen, Kaifeng and Eksombatchai, Pong and Hamilton, William L and Leskovec, Jure},
  booktitle={Proceedings of the 24th ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining},
  pages={974--983},
  year={2018}
}


@article{hu2020ogb,
  title={Open graph benchmark: Datasets for machine learning on graphs},
  author={Hu, Weihua and Fey, Matthias and Zitnik, Marinka and Dong, Yuxiao and Ren, Hongyu and Liu, Bowen and Catasta, Michele and Leskovec, Jure},
  journal={Advances in neural information processing systems},
  volume={33},
  pages={22118--22133},
  year={2020}
}

@article{hu2021ogblsc,
  title={OGB-LSC: A Large-Scale Challenge for Machine Learning on Graphs},
  author={Hu, Weihua and Fey, Matthias and Ren, Hongyu and Nakata, Maho and Dong, Yuxiao and Leskovec, Jure},
  journal={arXiv preprint arXiv:2103.09430},
  year={2021}
}

@inproceedings{hamilton2017inductive,
     author = {Hamilton, William L. and Ying, Rex and Leskovec, Jure},
     title = {Inductive Representation Learning on Large Graphs},
     booktitle = {NIPS},
     year = {2017}
   }

@article{wang2019dgl,
    title={Deep Graph Library: A Graph-Centric, Highly-Performant Package for Graph Neural Networks},
    author={Minjie Wang and Da Zheng and Zihao Ye and Quan Gan and Mufei Li and Xiang Song and Jinjing Zhou and Chao Ma and Lingfan Yu and Yu Gai and Tianjun Xiao and Tong He and George Karypis and Jinyang Li and Zheng Zhang},
    year={2019},
    journal={arXiv preprint arXiv:1909.01315}
}

@inproceedings{chiang_2019_clustergcn,
author = {Chiang, Wei-Lin and Liu, Xuanqing and Si, Si and Li, Yang and Bengio, Samy and Hsieh, Cho-Jui},
title = {Cluster-GCN: An Efficient Algorithm for Training Deep and Large Graph Convolutional Networks},
year = {2019},
booktitle = {Proceedings of the 25th ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining},
pages = {257–266},
numpages = {10},
keywords = {clustering, deep learning, graph convolutional networks, large-scale learning, semi-supervised learning},
series = {KDD '19}
}

@INPROCEEDINGS{graphsaint-ipdps19,
author={Hanqing Zeng and Hongkuan Zhou and Ajitesh Srivastava and Rajgopal Kannan and Viktor Prasanna},
booktitle={2019 IEEE International Parallel and Distributed Processing Symposium (IPDPS)},
title={Accurate, Efficient and Scalable Graph Embedding},
year={2019},
month={May},
}

@article{zheng_2022_distributed,
  author = {Zheng, Da and Song, Xiang and Yang, Chengru and LaSalle, Dominique and Karypis, George},
  month = {08},
  title = {Distributed Hybrid CPU and GPU training for Graph Neural Networks on Billion-Scale Heterogeneous Graphs},
  year = {2022},
  journal = {Proceedings of the 28th ACM SIGKDD Conference on Knowledge Discovery and Data Mining}
}

@article{karypis1997metis,
  title={METIS: A software package for partitioning unstructured graphs, partitioning meshes, and computing fill-reducing orderings of sparse matrices},
  author={Karypis, George and Kumar, Vipin},
  year={1997}
}

@article{yang_2023_betty,
  author = {Yang, Shuangyan and Zhang, Minjia and Dong, Wenqian and Li, Dong},
  title = {Betty: Enabling Large-Scale GNN Training with Batch-Level Graph Partitioning},
  year = {2023},
  journal = {Proceedings of the 28th ACM International Conference on Architectural Support for Programming Languages and Operating Systems}
}


@article{jia_improving_roc,
  title={Improving the accuracy, scalability, and performance of graph neural networks with roc},
  author={Jia, Zhihao and Lin, Sina and Gao, Mingyu and Zaharia, Matei and Aiken, Alex},
  journal={Proceedings of Machine Learning and Systems},
  volume={2},
  pages={187--198},
  year={2020}
}


@inproceedings{thorpe_dorylus,
  title={Dorylus: Affordable, scalable, and accurate $\{$GNN$\}$ training with distributed $\{$CPU$\}$ servers and serverless threads},
  author={Thorpe, John and Qiao, Yifan and Eyolfson, Jonathan and Teng, Shen and Hu, Guanzhou and Jia, Zhihao and Wei, Jinliang and Vora, Keval and Netravali, Ravi and Kim, Miryung and others},
  booktitle={15th USENIX Symposium on Operating Systems Design and Implementation (OSDI 21)},
  pages={495--514},
  year={2021}
}


@article{zou_2019_layerdependent,
  title={Layer-dependent importance sampling for training deep and large graph convolutional networks},
  author={Zou, Difan and Hu, Ziniu and Wang, Yewen and Jiang, Song and Sun, Yizhou and Gu, Quanquan},
  journal={Advances in neural information processing systems},
  volume={32},
  year={2019}
}


@misc{openai2020gpt3,
  author = {OpenAI},
  title = {Language Models are Unsupervised Multitask Learners},
  year = {2020},
  howpublished = {\url{https://cdn.openai.com/better-language-models/language_models_are_unsupervised_multitask_learners.pdf}},
  note = {Accessed: 22-05-2023}
}

@article{zitnik_2018_modeling,
	year = 2018,
	month = {jun},
  
	publisher = {Oxford University Press ({OUP})},
  
	volume = {34},
  
	number = {13},
  
	pages = {i457--i466},
  
	author = {Marinka Zitnik and Monica Agrawal and Jure Leskovec},
  
	title = {Modeling polypharmacy side effects with graph convolutional networks},
  
	journal = {Bioinformatics}
}

@inproceedings{schlichtkrull_modeling,
  title={Modeling relational data with graph convolutional networks},
  author={Schlichtkrull, Michael and Kipf, Thomas N and Bloem, Peter and Van Den Berg, Rianne and Titov, Ivan and Welling, Max},
  booktitle={The semantic web: 15th international conference, ESWC 2018, Heraklion, Crete, Greece, June 3--7, 2018, proceedings 15},
  pages={593--607},
  year={2018},
  organization={Springer}
}


@article{hamilton_embedding,
  title={Embedding logical queries on knowledge graphs},
  author={Hamilton, Will and Bajaj, Payal and Zitnik, Marinka and Jurafsky, Dan and Leskovec, Jure},
  journal={Advances in neural information processing systems},
  volume={31},
  year={2018}
}


@article{zhou_2020_graph,
  title={Graph neural networks: A review of methods and applications},
  author={Zhou, Jie and Cui, Ganqu and Hu, Shengding and Zhang, Zhengyan and Yang, Cheng and Liu, Zhiyuan and Wang, Lifeng and Li, Changcheng and Sun, Maosong},
  journal={AI open},
  volume={1},
  pages={57--81},
  year={2020},
  publisher={Elsevier}
}


@article{
  velikovi_graph,
  title="{Graph Attention Networks}",
  author={Veli{\v{c}}kovi{\'{c}}, Petar and Cucurull, Guillem and Casanova, Arantxa and Romero, Adriana and Li{\`{o}}, Pietro and Bengio, Yoshua},
  journal={International Conference on Learning Representations},
  year={2018},
  url={https://openreview.net/forum?id=rJXMpikCZ},
  note={accepted as poster},
}

@inproceedings{nextdoor,
  title={Accelerating Graph Sampling for Graph Machine Learning using GPUs},
  author={Jangda, Abhinav and Polisetty, Sandeep and Guha, Arjun and Serafini, Marco},
  booktitle={European Conference on Computer Systems (EuroSys)},
  year={2021}
}

@article{case-sampling,
author = {Serafini, Marco and Guan, Hui},
title = {Scalable Graph Neural Network Training: The Case for Sampling},
year = {2021},
issue_date = {July 2021},
volume = {55},
number = {1},
journal = {SIGOPS Oper. Syst. Rev.},
month = jun,
pages = {68–76}
}

@inproceedings{c-saw,
  title={C-SAW: A framework for graph sampling and random walk on GPUs},
  author={Pandey, Santosh and Li, Lingda and Hoisie, Adolfy and Li, Xiaoye S and Liu, Hang},
  booktitle={SC20: International Conference for High Performance Computing, Networking, Storage and Analysis},
  pages={1--15},
  year={2020},
  organization={IEEE}
}

@inproceedings{wang2021skywalker,
  title={Skywalker: Efficient Alias-Method-Based Graph Sampling and Random Walk on GPUs},
  author={Wang, Pengyu and Li, Chao and Wang, Jing and Wang, Taolei and Zhang, Lu and Leng, Jingwen and Chen, Quan and Guo, Minyi},
  booktitle={2021 30th International Conference on Parallel Architectures and Compilation Techniques (PACT)},
  pages={304--317},
  year={2021},
  organization={IEEE}
}


@inproceedings{kipf_semisupervised,
  title={Semi-Supervised Classification with Graph Convolutional Networks},
  author={Kipf, Thomas N. and Welling, Max},
  booktitle={International Conference on Learning Representations (ICLR)},
  year={2017}
}

@misc{_dgldataloadingmultilayerfullneighborsampler,
  author = {DGL},
  title = {dgl.dataloading.MultiLayerFullNeighborSampler — DGL 0.8.2post1 documentation},
  url = {https://docs.dgl.ai/en/0.8.x/generated/dgl.dataloading.MultiLayerFullNeighborSampler.html},
  urldate = {2023-10-14},
  organization = {docs.dgl.ai}
}

@misc{_reproducibility,
  author = {Pytorch},
  title = {Reproducibility — PyTorch 2.0 documentation},
  url = {https://pytorch.org/docs/stable/notes/randomness.html},
  organization = {pytorch.org}
}

@misc{mitson_2023_bayesian,
  author = {Mitson, Robert},
  month = {09},
  title = {Bayesian Hyperparameter Optimization - A Primer},
  url = {https://wandb.ai/site/articles/bayesian-hyperparameter-optimization-a-primer},
  urldate = {2023-10-14},
  year = {2023},
  organization = {W&B}
}

@misc{wandb_2022_tune,
  author = {wandb, },
  title = {Tune Hyperparameters - Documentation},
  url = {https://docs.wandb.ai/guides/sweeps},
  year = {2022},
  organization = {Wandb.ai}
}


@misc{dgl_2023_dmlcdgl,
  author = {dgl, dmlc},
  month = {10},
  title = {dmlc/dgl},
  url = {https://github.com/dmlc/dgl/tree/master},
  urldate = {2023-10-14},
  year = {2023},
  organization = {GitHub}
}

@misc{pipegcngtihub_2023_pipegcn,
  author={Wan, C and Li, Y and Wolfe, Cameron R and Kyrillidis, A and Kim, Nam S and Lin, Y},
  title = {PipeGCN repository},
  url = {https://github.com/GATECH-EIC/PipeGCN},
  urldate = {2023-10-14},
  year = {2023},
  organization = {GitHub}
}


@misc{mini-vs-full-extended,
  author = {Saurabh Bajaj and Hoaje Son and Juelin Liu and Hui Guan and Marco Serafini},
  title = {Graph Neural Network Training Systems: A Comparison of Full-Graph and Mini-Batch - Extended Version},
  url = {https://github.com/saurabhbajaj123/GNN\_minibatch\_vs\_fullbatch},
  year = 2024
}

@misc{quiver_2023_quiverteamtorchquiver,
  author = {Quiver},
  month = {10},
  title = {quiver-team/torch-quiver},
  url = {https://github.com/quiver-team/torch-quiver},
  urldate = {2023-10-15},
  year = {2023},
  organization = {GitHub}
}

@misc{bns-gcn-repo,
  author = {Cheng Wan and Youjie Li and Ang Li and Nam Sung Kim and Yingyan Lin},
  title = {BNS-GCN repository},
  url = {https://github.com/GATECH-EIC/BNS-GCN},
  year = 2023
}

@misc{adaqp-repo,
  author = {Borui Wan and Juntao Zhao and Chuan Wu},
  title = {AdaQP repository},
  url = {https://github.com/raywan-110/AdaQP},
  year = 2024
}

@misc{mini-full-repo2,
  author = {Saurabh Bajaj and Hojae Son and Juelin Liu and Hui Guan and Marco Serafini},
  title = {Graph Neural Network Training Systems: A Performance
Comparison of Full-Graph and Mini-Batch. Repository},
  url = {https://github.com/saurabhbajaj123/GNN_minibatch_vs_fullbatch},
  year = 2024
}



@misc{tan_quiver,
    author = {Zeyuan Tan and Xiulong Yuan and Congjie He and Man-Kit Sit and Guo Li and Xiaoze Liu and Baole Ai and Kai Zeng and Peter Pietzuch and Luo Mai},
    title = {Quiver: Supporting GPUs for Low-Latency, High-Throughput GNN Serving with Workload Awareness},
    eprint={2305.10863},
    year = {2023}
}



@inproceedings{xu_optimization,
  title={Optimization of graph neural networks: Implicit acceleration by skip connections and more depth},
  author={Xu, Keyulu and Zhang, Mozhi and Jegelka, Stefanie and Kawaguchi, Kenji},
  booktitle={International Conference on Machine Learning},
  pages={11592--11602},
  year={2021},
  organization={PMLR}
}

@article{chen_2022_learning,
  author = {Chen, Yihao and Tang, Xin and Qi, Xianbiao and Li, Chun-Guang and Xiao, Rong},
  month = {01},
  title = {Learning graph normalization for graph neural networks},
  doi = {10.1016/j.neucom.2022.01.003},
  urldate = {2022-03-06},
  year = {2022},
  journal = {Neurocomputing}
}


@misc{pygvsdgl_pytorch,
  author = {PyGvsDGL, },
  title = {PyTorch Geometric vs Deep Graph Library},
  url = {https://www.exxactcorp.com/blog/Deep-Learning/pytorch-geometric-vs-deep-graph-library},
  urldate = {2023-10-19},
  organization = {www.exxactcorp.com}
}

@misc{song_2021_network,
  author = {{Song, Xiang and Aws, A and Usa, Runjie and Ma,  and Shanghai, Aws and Lab, A and Li, China and Zhang, Muhan and David Wipf}},
  title = {Network In Graph Neural Network},
  url = {https://arxiv.org/pdf/2111.11638.pdf},
  urldate = {2023-10-21},
  year = {2021}
}


@misc{rusch_a,
      title={A Survey on Oversmoothing in Graph Neural Networks}, 
      author={T. Konstantin Rusch and Michael M. Bronstein and Siddhartha Mishra},
      year={2023},
      eprint={2303.10993},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@inproceedings{wan_pipegcn,
  title={{PipeGCN}: Efficient Full-Graph Training of Graph Convolutional Networks with Pipelined Feature Communication},
  author={Wan, C and Li, Y and Wolfe, Cameron R and Kyrillidis, A and Kim, Nam S and Lin, Y},
  booktitle={The Tenth International Conference on Learning Representations (ICLR 2022)},
  year={2022}
}


@inproceedings{Ying_2018,
	author = {Rex Ying and Ruining He and Kaifeng Chen and Pong Eksombatchai and William L. Hamilton and Jure Leskovec},
	title = {Graph Convolutional Neural Networks for Web-Scale Recommender Systems},
	booktitle = {Proceedings of the 24th {ACM} {SIGKDD} International Conference on Knowledge Discovery {\&}amp$\mathsemicolon$ Data Mining},
    year = {2018}
}


@inproceedings{Krzywda_2022,
	doi = {10.1109/ijcnn55064.2022.9892658},
	url = {https://doi.org/10.1109%2Fijcnn55064.2022.9892658},
	year = 2022,
	month = {jul},
	publisher = {{IEEE}
},
	author = {Maciej Krzywda and Szymon Lukasik and Amir H. Gandomi},
	title = {Graph Neural Networks in Computer Vision - Architectures, Datasets and Common Approaches},
	booktitle = {2022 International Joint Conference on Neural Networks ({IJCNN})}
}

@article{wu2022graph,
  title={Graph neural networks for natural language processing: A survey},
  author={Wu, Lingfei and Chen, Yu and Shen, Kai and Guo, Xiaojie and Gao, Hanning and Li, Shucheng and Pei, Jian and Long, Bo and others},
  journal={Foundations and Trends{\textregistered} in Machine Learning},
  volume={16},
  number={2},
  pages={119--328},
  year={2023},
  publisher={Now Publishers, Inc.}
}


@article{Wu_2021,
	doi = {10.1109/tnnls.2020.2978386},
	url = {https://doi.org/10.1109%2Ftnnls.2020.2978386},
	year = 2021,
	month = {jan},
	publisher = {Institute of Electrical and Electronics Engineers ({IEEE})},
	volume = {32},
	number = {1},
	pages = {4--24},
	author = {Zonghan Wu and Shirui Pan and Fengwen Chen and Guodong Long and Chengqi Zhang and Philip S. Yu},
	title = {A Comprehensive Survey on Graph Neural Networks},
	journal = {{IEEE} Transactions on Neural Networks and Learning Systems}
}

@inproceedings{md2021distgnn,
  title={Distgnn: Scalable distributed training for large-scale graph neural networks},
  author={Md, Vasimuddin and Misra, Sanchit and Ma, Guixiang and Mohanty, Ramanarayan and Georganas, Evangelos and Heinecke, Alexander and Kalamkar, Dhiraj and Ahmed, Nesreen K and Avancha, Sasikanth},
  booktitle={Proceedings of the International Conference for High Performance Computing, Networking, Storage and Analysis},
  pages={1--14},
  year={2021}
}

@inproceedings{zheng2021distdgl,
  title={Distdgl: distributed graph neural network training for billion-scale graphs},
  author={Zheng, Da and Ma, Chao and Wang, Minjie and Zhou, Jinjing and Su, Qidong and Song, Xiang and Gan, Quan and Zhang, Zheng and Karypis, George},
  booktitle={2020 IEEE/ACM 10th Workshop on Irregular Applications: Architectures and Algorithms (IA3)},
  pages={36--44},
  year={2020},
  organization={IEEE}
}


@misc{chen2023gnnpipe,
      title={GNNPipe: Scaling Deep GNN Training with Pipelined Model Parallelism}, 
      author={Jingji Chen and Zhuoming Chen and Xuehai Qian},
      year={2023},
      eprint={2308.10087},
      archivePrefix={arXiv},
      primaryClass={cs.DC}
}

@inproceedings {wang2023mgg,
author = {Yuke Wang and Boyuan Feng and Zheng Wang and Tong Geng and Kevin Barker and Ang Li and Yufei Ding},
title = {{MGG}: Accelerating Graph Neural Networks with {Fine-Grained} {Intra-Kernel} {Communication-Computation} Pipelining on {Multi-GPU} Platforms},
booktitle = {17th USENIX Symposium on Operating Systems Design and Implementation (OSDI 23)},
year = {2023},
isbn = {978-1-939133-34-2},
address = {Boston, MA},
pages = {779--795},
url = {https://www.usenix.org/conference/osdi23/presentation/wang-yuke},
publisher = {USENIX Association},
month = jul
}

@article{wan2022bnsgcn,
  title={{BNS-GCN}: Efficient Full-graph Training of Graph Convolutional Networks with Partition-parallelism and Random Boundary Node Sampling},
  author={Wan, Cheng and Li, Youjie and Li, Ang and Kim, Nam Sung and Lin, Yingyan},
  journal={Proceedings of Machine Learning and Systems},
  volume={4},
  pages={673--693},
  year={2022}
}

@article{mostafa2022sequential,
  title={Sequential Aggregation and Rematerialization: Distributed Full-batch Training of Graph Neural Networks on Large Graphs},
  author={Mostafa, Hesham},
  journal={MLSys},
  year={2022}
}

@inproceedings{namata:mlg12,
  title={Query-driven active surveying for collective classification},
  author={Namata, Galileo and London, Ben and Getoor, Lise and Huang, Bert and Edu, U},
  booktitle={10th international workshop on mining and learning with graphs},
  volume={8},
  pages={1},
  year={2012}
}


@article{song2023adgnn,
  title={ADGNN: Towards Scalable GNN Training with Aggregation-Difference Aware Sampling},
  author={Song, Zhen and Gu, Yu and Li, Tianyi and Sun, Qing and Zhang, Yanfeng and Jensen, Christian S and Yu, Ge},
  journal={Proceedings of the ACM on Management of Data},
  volume={1},
  number={4},
  pages={1--26},
  year={2023},
  publisher={ACM New York, NY, USA}
}

@article{wang2023hongtu,
  title={HongTu: Scalable Full-Graph GNN Training on Multiple GPUs},
  author={Wang, Qiange and Chen, Yao and Wong, Weng-Fai and He, Bingsheng},
  journal={Proceedings of the ACM on Management of Data},
  volume={1},
  number={4},
  pages={1--27},
  year={2023},
  publisher={ACM New York, NY, USA}
}

@article{Yang2022WholeGraphAF,
  title={WholeGraph: A Fast Graph Neural Network Training Framework with Multi-GPU Distributed Shared Memory Architecture},
  author={Dongxu Yang and Junhong Liu and Jiaxing Qi and Junjie Lai},
  journal={SC22: International Conference for High Performance Computing, Networking, Storage and Analysis},
  year={2022},
  pages={1-14}
}

@inproceedings{zhou2022gnnear,
  title={Gnnear: Accelerating full-batch training of graph neural networks with near-memory processing},
  author={Zhou, Zhe and Li, Cong and Wei, Xuechao and Wang, Xiaoyang and Sun, Guangyu},
  booktitle={Proceedings of the International Conference on Parallel Architectures and Compilation Techniques},
  pages={54--68},
  year={2022}
}


@InProceedings{you2020design,
  title = {Design Space for Graph Neural Networks},
  author = {You, Jiaxuan and Ying, Rex and Leskovec, Jure},
  booktitle = {NeurIPS},
  year = {2020}
}


@article{G3_full_graph,
author = {Wan, Xinchen and Xu, Kaiqiang and Liao, Xudong and Jin, Yilun and Chen, Kai and Jin, Xin},
title = {Scalable and Efficient Full-Graph GNN Training for Large Graphs},
year = {2023},
volume = {1},
number = {2},
journal = {Proc. ACM Manag. Data},
keywords = {distributed training, hybrid parallelism, GPU, graph neural network}
}

@article{lin_2020_pagraph,
  author = {Lin, Zhiqi and Li, Cheng and Miao, Youshan and Liu, Yunxin and Xu, Yinlong},
  month = {10},
  title = {{PaGraph}: Scaling {GNN} training on large graphs via computation-aware caching},
  doi = {10.1145/3419111.3421281},
  year = {2020},
  journal = {Proceedings of the 11th ACM Symposium on Cloud Computing}
}

@inproceedings{DBLP_tripathy_cagnet,
  title={Reducing communication in graph neural network training},
  author={Tripathy, Alok and Yelick, Katherine and Bulu{\c{c}}, Ayd{\i}n},
  booktitle={SC20: International Conference for High Performance Computing, Networking, Storage and Analysis},
  pages={1--14},
  year={2020},
  organization={IEEE}
}


@inproceedings{ugache,
author = {Song, Xiaoniu and Zhang, Yiwen and Chen, Rong and Chen, Haibo},
title = {UGACHE: A Unified GPU Cache for Embedding-Based Deep Learning},
year = {2023},
booktitle = {Proceedings of the 29th Symposium on Operating Systems Principles},
pages = {627–641},
numpages = {15},
keywords = {GPU cache, GPU interconnect, embedding},
series = {SOSP '23}
}


@inproceedings{liu_exact,
  title={Exact: Scalable graph neural networks training via extreme activation compression},
  author={Liu, Zirui and Zhou, Kaixiong and Yang, Fan and Li, Li and Chen, Rui and Hu, Xia},
  booktitle={International Conference on Learning Representations},
  year={2021}
}

@inproceedings {ma_neugraph,
author = {Lingxiao Ma and Zhi Yang and Youshan Miao and Jilong Xue and Ming Wu and Lidong Zhou and Yafei Dai},
title = {{NeuGraph}: Parallel Deep Neural Network Computation on Large Graphs},
booktitle = {2019 USENIX Annual Technical Conference (USENIX ATC 19)},
year = {2019},
pages = {443--458},
month = jul
}


@article{wang_2022_neutronstar,
  author = {Wang, Qiange and Zhang, Yanfeng and Wang, Hao and Chen, Chaoyi and Zhang, Xiaodong and Yu, Ge},
  month = {06},
  title = {NeutronStar: Distributed GNN Training with Hybrid Dependency Management},
  year = {2022},
  journal = {Proceedings of the 2022 International Conference on Management of Data}
}

@inproceedings{cai_2021_dgcl,
  title={DGCL: An efficient communication library for distributed GNN training},
  author={Cai, Zhenkun and Yan, Xiao and Wu, Yidi and Ma, Kaihao and Cheng, James and Yu, Fan},
  booktitle={Proceedings of the Sixteenth European Conference on Computer Systems},
  pages={130--144},
  year={2021}
}


@article{wan2023adaptive,
  title={Adaptive message quantization and parallelization for distributed full-graph {GNN} training},
  author={Wan, Borui and Zhao, Juntao and Wu, Chuan},
  journal={Proceedings of Machine Learning and Systems},
  volume={5},
  year={2023}
}


@article{shao2023distributed,
  title={Distributed graph neural network training: A survey},
  author={Shao, Yingxia and Li, Hongzheng and Gu, Xizhi and Yin, Hongbo and Li, Yawen and Miao, Xupeng and Zhang, Wentao and Cui, Bin and Chen, Lei},
  journal={ACM Computing Surveys},
  volume={56},
  number={8},
  pages={1--39},
  year={2024},
  publisher={ACM New York, NY}
}

@article{Vatter_2023,
   title={The Evolution of Distributed Systems for Graph Neural Networks and Their Origin in Graph Processing and Deep Learning: A Survey},
   volume={56},
   ISSN={1557-7341},
   url={http://dx.doi.org/10.1145/3597428},
   DOI={10.1145/3597428},
   number={1},
   journal={ACM Computing Surveys},
   publisher={Association for Computing Machinery (ACM)},
   author={Vatter, Jana and Mayer, Ruben and Jacobsen, Hans-Arno},
   year={2023},
   month=aug, pages={1–37} }



@article{lin2023comprehensive,
  title={A comprehensive survey on distributed training of graph neural networks},
  author={Lin, Haiyang and Yan, Mingyu and Ye, Xiaochun and Fan, Dongrui and Pan, Shirui and Chen, Wenguang and Xie, Yuan},
  journal={Proceedings of the IEEE},
  year={2023},
  publisher={IEEE}
}


@inproceedings{liu2023bgl,
  title={{BGL}: {GPU}-Efficient {GNN} Training by Optimizing Graph Data {I/O} and Preprocessing},
  author={Liu, Tianfeng and Chen, Yangrui and Li, Dan and Wu, Chuan and Zhu, Yibo and He, Jun and Peng, Yanghua and Chen, Hongzheng and Chen, Hongzhi and Guo, Chuanxiong},
  booktitle={20th USENIX Symposium on Networked Systems Design and Implementation (NSDI 23)},
  pages={103--118},
  year={2023}
}


@article{comprehensive-gnn,
author = {Yuan, Hao and Liu, Yajiong and Zhang, Yanfeng and Ai, Xin and Wang, Qiange and Chen, Chaoyi and Gu, Yu and Yu, Ge},
title = {Comprehensive Evaluation of GNN Training Systems: A Data Management Perspective},
year = {2024},
issue_date = {February 2024},
publisher = {VLDB Endowment},
volume = {17},
number = {6},
issn = {2150-8097},
journal = {Proc. VLDB Endow.},
month = {may},
pages = {1241–1254},
numpages = {14}
}

@article{gsplit-arxiv,
  title={GSplit: Scaling Graph Neural Network Training on Large Graphs via Split-Parallelism},
  author={Polisetty, Sandeep and Liu, Juelin and Falus, Kobi and Fung, Yi Ren and Lim, Seung-Hwan and Guan, Hui and Serafini, Marco},
  journal={arXiv preprint arXiv:2303.13775},
  month={Mar.},
  year={2023}
}

@inproceedings{yang_gnnlab,
author = {Yang, Jianbang and Tang, Dahai and Song, Xiaoniu and Wang, Lei and Yin, Qiang and Chen, Rong and Yu, Wenyuan and Zhou, Jingren},
title = {GNNLab: A Factored System for Sample-Based GNN Training over GPUs},
year = {2022},
booktitle = {Proceedings of the Seventeenth European Conference on Computer Systems},
pages = {417–434},
keywords = {sample-based GNN training, caching policy, graph neural networks},
series = {EuroSys '22}
}

@inproceedings{dsp_cai,
author = {Cai, Zhenkun and Zhou, Qihui and Yan, Xiao and Zheng, Da and Song, Xiang and Zheng, Chenguang and Cheng, James and Karypis, George},
title = {DSP: Efficient GNN Training with Multiple GPUs},
year = {2023},
booktitle = {Proceedings of the 28th ACM SIGPLAN Annual Symposium on Principles and Practice of Parallel Programming},
pages = {392–404},
numpages = {13},
keywords = {graph neural networks, GPU, model training},
series = {PPoPP '23}
}

@inproceedings {legion_sun,
author = {Jie Sun and Li Su and Zuocheng Shi and Wenting Shen and Zeke Wang and Lei Wang and Jie Zhang and Yong Li and Wenyuan Yu and Jingren Zhou and Fei Wu},
title = {Legion: Automatically Pushing the Envelope of {Multi-GPU} System for {Billion-Scale} {GNN} Training},
booktitle = {2023 USENIX Annual Technical Conference (USENIX ATC 23)},
year = {2023},
pages = {165--179}
}

@inproceedings {p3_gandhi,
author = {Swapnil Gandhi and Anand Padmanabha Iyer},
title = {P3: Distributed Deep Graph Learning at Scale},
booktitle = {15th {USENIX} Symposium on Operating Systems Design and Implementation ({OSDI} 21)},
year = {2021},
pages = {551--568},
month = jul
}


@article{zhu2019aligraph,
  title={AliGraph: a comprehensive graph neural network platform},
  author={Zhu, Rong and Zhao, Kun and Yang, Hongxia and Lin, Wei and Zhou, Chang and Ai, Baole and Li, Yong and Zhou, Jingren},
  journal={Proceedings of the VLDB Endowment},
  volume={12},
  number={12},
  pages={2094--2105},
  year={2019},
  publisher={VLDB Endowment}
}

@INPROCEEDINGS{cm_gcn_zhao,
  author={Zhao, Guoyi and Zhou, Tian and Gao, Lixin},
  booktitle={2021 IEEE International Conference on Big Data (Big Data)}, 
  title={CM-GCN: A Distributed Framework for Graph Convolutional Networks using Cohesive Mini-batches}, 
  year={2021},
  volume={},
  number={},
  pages={153-163},
  doi={10.1109/BigData52589.2021.9671931}}


@article{byteGCN_zheng,
author = {Zheng, Chenguang and Chen, Hongzhi and Cheng, Yuxuan and Song, Zhezheng and Wu, Yifan and Li, Changji and Cheng, James and Yang, Hao and Zhang, Shuai},
title = {ByteGNN: Efficient Graph Neural Network Training at Large Scale},
year = {2022},
issue_date = {February 2022},
publisher = {VLDB Endowment},
volume = {15},
number = {6},
issn = {2150-8097},
url = {https://doi.org/10.14778/3514061.3514069},
doi = {10.14778/3514061.3514069},
journal = {Proc. VLDB Endow.},
month = {feb},
pages = {1228–1242},
numpages = {15}
}

@article{zhang2020agl,
    author = {Zhang, Dalong and Huang, Xin and Liu, Ziqi and Zhou, Jun and Hu, Zhiyang and Song, Xianzheng and Ge, Zhibang and Wang, Lin and Zhang, Zhiqiang and Qi, Yuan},
    title = {AGL: a scalable system for industrial-purpose graph machine learning},
    year = {2020},
    volume = {13},
    number = {12},
    journal = {Proc. VLDB Endow.},
    pages = {3125–3137}
}

@Inproceedings{gsampler,
 author = {Ping Gong and Renjie Liu and Zunyao Mao and Zhenkun Cai and Xiao Yan and Cheng Li and Minjie Wang and Zhuozhao Li},
 title = {gSampler: General and efficient GPU-based graph sampling for graph learning},
 year = {2023},
 booktitle = {ACM 2023 Symposium on Operating Systems Principles (SOSP)},
}

@article{sancus,
author = {Peng, Jingshu and Chen, Zhao and Shao, Yingxia and Shen, Yanyan and Chen, Lei and Cao, Jiannong},
title = {Sancus: staleness-aware communication-avoiding full-graph decentralized training in large-scale graph neural networks},
year = {2022},
issue_date = {May 2022},
publisher = {VLDB Endowment},
volume = {15},
number = {9},
journal = {Proc. VLDB Endow.},
pages = {1937–1950},
}

@inproceedings{pipedream,
author = {Narayanan, Deepak and Harlap, Aaron and Phanishayee, Amar and Seshadri, Vivek and Devanur, Nikhil R. and Ganger, Gregory R. and Gibbons, Phillip B. and Zaharia, Matei},
title = {PipeDream: generalized pipeline parallelism for DNN training},
year = {2019},
isbn = {9781450368735},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3341301.3359646},
doi = {10.1145/3341301.3359646},
booktitle = {Proceedings of the 27th ACM Symposium on Operating Systems Principles},
pages = {1–15},
numpages = {15},
location = {Huntsville, Ontario, Canada},
series = {SOSP '19}
}

@article{single_cell_rna,
title = {Imputing single-cell RNA-seq data by combining graph convolution and autoencoder neural networks},
journal = {iScience},
volume = {24},
number = {5},
pages = {102393},
year = {2021},
issn = {2589-0042},
doi = {https://doi.org/10.1016/j.isci.2021.102393},
url = {https://www.sciencedirect.com/science/article/pii/S2589004221003618},
author = {Jiahua Rao and Xiang Zhou and Yutong Lu and Huiying Zhao and Yuedong Yang},
keywords = {Genomics, Bioinformatics, Data Acquisition in Bioinformatics, Artificial Intelligence},
}



@article{demirci2022scalable_parallelgcn,
author = {Demirci, Gunduz Vehbi and Haldar, Aparajita and Ferhatosmanoglu, Hakan},
title = {Scalable Graph Convolutional Network Training on Distributed-Memory Systems},
year = {2022},
volume = {16},
number = {4},
journal = {Proc. VLDB Endow.},
month = {dec},
pages = {711–724},
numpages = {14}
}


@inproceedings{yang2012defining_snap,
  title={Defining and evaluating network communities based on ground-truth},
  author={Yang, Jaewon and Leskovec, Jure},
  booktitle={Proceedings of the ACM SIGKDD Workshop on Mining Data Semantics},
  pages={1--8},
  year={2012}
}


@misc{chen2018fastgcn,
      title={FastGCN: Fast Learning with Graph Convolutional Networks via Importance Sampling}, 
      author={Jie Chen and Tengfei Ma and Cao Xiao},
      year={2018},
      eprint={1801.10247},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}


@article{ai2023neutronorch,
  title={NeutronOrch: Rethinking Sample-based GNN Training under CPU-GPU Heterogeneous Environments},
  author={Ai, Xin and Wang, Qiange and Cao, Chunyu and Zhang, Yanfeng and Chen, Chaoyi and Yuan, Hao and Gu, Yu and Yu, Ge},
  journal={arXiv preprint arXiv:2311.13225},
  year={2023}
}

@INPROCEEDINGS{rdm,
  author={Kurt, Süreyya Emre and Yan, Jinghua and Sukumaran-Rajam, Aravind and Pandey, Prashant and Sadayappan, P.},
  booktitle={2023 IEEE International Parallel and Distributed Processing Symposium (IPDPS)}, 
  title={Communication Optimization for Distributed Execution of Graph Neural Networks}, 
  year={2023},
  volume={},
  number={},
  pages={512-523},
  keywords={Training;Distributed processing;Machine learning algorithms;Machine learning;Graph neural networks;Partitioning algorithms;Sparse matrices;Graph Neural Networks;Distributed Algorithms;Multi-GPU GNN;Performance Modeling},
  doi={10.1109/IPDPS54959.2023.00058}}


@article{liu2021sampling,
  title={Sampling methods for efficient training of graph convolutional networks: A survey},
  author={Liu, Xin and Yan, Mingyu and Deng, Lei and Li, Guoqi and Ye, Xiaochun and Fan, Dongrui},
  journal={IEEE/CAA Journal of Automatica Sinica},
  volume={9},
  number={2},
  pages={205--234},
  year={2021},
  publisher={IEEE}
}


@inproceedings{li2024rethinking,
author = {Li, Xunkai and Ma, Jingyuan and Wu, Zhengyu and Su, Daohan and Zhang, Wentao and Li, Rong-Hua and Wang, Guoren},
title = {Rethinking Node-wise Propagation for Large-scale Graph Learning},
year = {2024},
booktitle = {Proceedings of the ACM on Web Conference 2024},
pages = {560–569},
numpages = {10},
keywords = {graph neural networks, scalability, semi-supervised learning},
series = {WWW '24}
}


@InProceedings{pmlr-v198-gasteiger22a_influence_based,
  title = 	 {Influence-Based Mini-Batching for Graph Neural Networks},
  author =       {Gasteiger, Johannes and Qian, Chendi and G{\"u}nnemann, Stephan},
  booktitle = 	 {Proceedings of the First Learning on Graphs Conference},
  pages = 	 {9:1--9:19},
  year = 	 {2022},
  volume = 	 {198},
  series = 	 {Proceedings of Machine Learning Research},
  month = 	 {09--12 Dec},
}


@article{hoang2021efficient_deepgalois,
  title={Efficient distribution for deep learning on large graphs},
  author={Hoang, Loc and Chen, Xuhao and Lee, Hochan and Dathathri, Roshan and Gill, Gurbinder and Pingali, Keshav},
  journal={update},
  volume={1050},
  pages={1},
  year={2021}
}




@article{kaler2022accelerating_salient,
  title={Accelerating training and inference of graph neural networks with fast sampling and pipelining},
  author={Kaler, Tim and Stathas, Nickolas and Ouyang, Anne and Iliopoulos, Alexandros-Stavros and Schardl, Tao and Leiserson, Charles E and Chen, Jie},
  journal={Proceedings of Machine Learning and Systems},
  volume={4},
  pages={172--189},
  year={2022}
}

@article{kaler2023communicationefficient_salient++,
  title={Communication-efficient graph neural networks with probabilistic neighborhood expansion analysis and caching},
  author={Kaler, Tim and Iliopoulos, Alexandros and Murzynowski, Philip and Schardl, Tao and Leiserson, Charles E and Chen, Jie},
  journal={Proceedings of Machine Learning and Systems},
  volume={5},
  year={2023}
}

@misc{chen2018stochastic_vrgcn,
      title={Stochastic Training of Graph Convolutional Networks with Variance Reduction}, 
      author={Jianfei Chen and Jun Zhu and Le Song},
      year={2018},
      eprint={1710.10568},
      archivePrefix={arXiv},
      primaryClass={stat.ML}
}

@article{huang2018adaptive_sgcn,
  title={Adaptive sampling towards fast graph representation learning},
  author={Huang, Wenbing and Zhang, Tong and Rong, Yu and Huang, Junzhou},
  journal={Advances in neural information processing systems},
  volume={31},
  year={2018}
}


@inproceedings{yao2021blocking,
  title={Blocking-based Neighbor Sampling for Large-scale Graph Neural Networks.},
  author={Yao, Kai-Lang and Li, Wu-Jun},
  booktitle={IJCAI},
  pages={3307--3313},
  year={2021}
}

@article{wu2024sgformer,
  title={Simplifying and empowering transformers for large-graph representations},
  author={Wu, Qitian and Zhao, Wentao and Yang, Chenxiao and Zhang, Hengrui and Nie, Fan and Jiang, Haitian and Bian, Yatao and Yan, Junchi},
  journal={Advances in Neural Information Processing Systems},
  volume={36},
  year={2024}
}




@inproceedings{frasca2020sign,
    title={SIGN: Scalable Inception Graph Neural Networks},
    author={Fabrizio Frasca and Emanuele Rossi and Davide Eynard and Benjamin Chamberlain and Michael Bronstein and Federico Monti},
    booktitle={ICML 2020 Workshop on Graph Representation Learning and Beyond},
    year={2020}
}









%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%












@ARTICLE{EfficientDataLoader,
  author={Bai, Youhui and Li, Cheng and Lin, Zhiqi and Wu, Yufei and Miao, Youshan and Liu, Yunxin and Xu, Yinlong},
  journal={IEEE Transactions on Parallel and Distributed Systems}, 
  title={Efficient Data Loader for Fast Sampling-Based GNN Training on Large Graphs}, 
  year={2021},
  volume={32},
  number={10},
  pages={2541-2556},
  keywords={Training;Graphics processing units;Loading;Computational modeling;Load modeling;Partitioning algorithms;Deep learning;Graph neural network;cache;large graph;graph partition;pipeline;multi-GPU}
}

@article{deutsch2019tigergraph,
  title={Tigergraph: A native MPP graph database},
  author={Deutsch, Alin and Xu, Yu and Wu, Mingxi and Lee, Victor},
  journal={arXiv preprint arXiv:1901.08248},
  year={2019}
}

@inproceedings{dong2021global,
  title={Global neighbor sampling for mixed CPU-GPU training on giant graphs},
  author={Dong, Jialin and Zheng, Da and Yang, Lin F and Karypis, George},
  booktitle={Proceedings of the 27th ACM SIGKDD Conference on Knowledge Discovery \& Data Mining},
  pages={289--299},
  year={2021}
}


@article{Largegraphconvolutional,
author = {Min, Seung Won and Wu, Kun and Huang, Sitao and Hidayeto\u{g}lu, Mert and Xiong, Jinjun and Ebrahimi, Eiman and Chen, Deming and Hwu, Wen-mei},
title = {Large graph convolutional network training with GPU-oriented data communication architecture},
year = {2021},
issue_date = {July 2021},
publisher = {VLDB Endowment},
volume = {14},
number = {11},
journal = {Proc. VLDB Endow.},
month = {jul},
pages = {2087–2100},
numpages = {14}
}

@article{DUCATI,
  title={DUCATI: A Dual-Cache Training System for Graph Neural Networks on Giant Graphs with the GPU},
  author={Zhang, Xin and Shen, Yanyan and Shao, Yingxia and Chen, Lei},
  journal={Proceedings of the ACM on Management of Data},
  volume={1},
  number={2},
  pages={1--24},
  year={2023},
  publisher={ACM New York, NY, USA}
}

@article{kaler2023communication,
  title={Communication-efficient graph neural networks with probabilistic neighborhood expansion analysis and caching},
  author={Kaler, Tim and Iliopoulos, Alexandros and Murzynowski, Philip and Schardl, Tao and Leiserson, Charles E and Chen, Jie},
  journal={Proceedings of Machine Learning and Systems},
  volume={5},
  year={2023}
}


@article{jiang2021communication,
  title={Communication-efficient sampling for distributed training of graph convolutional networks},
  author={Jiang, Peng and Rumi, Masuma Akter},
  journal={arXiv preprint arXiv:2101.07706},
  year={2021}
}

@inproceedings{yang2019knightking,
  title={Knightking: a fast distributed graph random walk engine},
  author={Yang, Ke and Zhang, MingXing and Chen, Kang and Ma, Xiaosong and Bai, Yang and Jiang, Yong},
  booktitle={Proceedings of the 27th ACM symposium on operating systems principles},
  pages={524--537},
  year={2019}
}



@inproceedings{ramezani2021learn,
  title={Learn Locally, Correct Globally: A Distributed Algorithm for Training Graph Neural Networks},
  author={Ramezani, Morteza and Cong, Weilin},
  booktitle={International Conference on Learning (ICLR)},
  year={2022}
}

@article{liu2021graphtheta,
  title={GraphTheta: A distributed graph neural network learning system with flexible training strategy},
  author={Liu, Yongchao and Li, Houyi and Zhang, Guowei and Zeng, Xintan and Li, Yongyong and Huang, Bin and Zhang, Peng and Li, Zhao and Zhu, Xiaowei and He, Changhua and others},
  journal={arXiv preprint arXiv:2104.10569},
  year={2021}
}

@article{xue2023sugar,
  title={SUGAR: Efficient Subgraph-level Training via Resource-aware Graph Partitioning},
  author={Xue, Zihui and Yang, Yuedong and Marculescu, Radu},
  journal={IEEE Transactions on Computers},
  year={2023},
  publisher={IEEE}
}

@article{zhao2023distributed,
  title={Distributed optimization of graph convolutional network using subgraph variance},
  author={Zhao, Taige and Song, Xiangyu and Li, Man and Li, Jianxin and Luo, Wei and Razzak, Imran},
  journal={IEEE Transactions on Neural Networks and Learning Systems},
  year={2023},
  publisher={IEEE}
}

@article{angerd2020distributed,
  title={Distributed training of graph convolutional networks using subgraph approximation},
  author={Angerd, Alexandra and Balasubramanian, Keshav and Annavaram, Murali},
  journal={arXiv preprint arXiv:2012.04930},
  year={2020}
}


@inproceedings{jangda2021accelerating,
  title={Accelerating graph sampling for graph machine learning using GPUs},
  author={Jangda, Abhinav and Polisetty, Sandeep and Guha, Arjun and Serafini, Marco},
  booktitle={Proceedings of the sixteenth European conference on computer systems},
  pages={311--326},
  year={2021}
}



@inproceedings{wang2021flexgraph,
  title={FlexGraph: a flexible and efficient distributed framework for GNN training},
  author={Wang, Lei and Yin, Qiang and Tian, Chao and Yang, Jianbang and Chen, Rong and Yu, Wenyuan and Yao, Zihang and Zhou, Jingren},
  booktitle={Proceedings of the Sixteenth European Conference on Computer Systems},
  pages={67--82},
  year={2021}
}

@inproceedings{min2022graph,
  title={Graph neural network training and data tiering},
  author={Min, Seung Won and Wu, Kun and Hidayetoglu, Mert and Xiong, Jinjun and Song, Xiang and Hwu, Wen-mei},
  booktitle={Proceedings of the 28th ACM SIGKDD Conference on Knowledge Discovery and Data Mining},
  pages={3555--3565},
  year={2022}
}



==> sections/21-CPU-evaluation.tex <==
\spara{CPU-based evaluation.} To further confirm the gap in computation cost in a hardware-independent manner, we run both full-graph and mini-batch training on the same training system, DGL, in the same CPU-based setting where all training data is stored in the main memory.
We use a host equipped with 2 Intel(R) Xeon(R) Gold 6240 CPU @ 2.60GHz with 28 cores each and 184GB of host memory.

Figure~\ref{fig:mb_vs_full_cpu} compares the results for single CPU host training with GraphSage. On arxiv, reddit, and ogbn-products, we observe that the mini-batch training implementation converges faster than the full-graph training implementation. Even though mini-batch system has longer epoch times, it requires less number of epochs to reach optimal accuracy and hence shorter time-to-accuracy. This observation is aligned with our training cost analysis, which shows that mini-batch training converge faster because it requires less computation. 

% Table~\ref{tab:cpu_epoch_tta} further reports the breakdown of the epoch time. For mini-batch training system, when using a larger number of sampling layers and fanouts, the forward and backward time dominate the epoch time (Ogbn-Products). However, the when using fewer sampling layers and small fanouts, sampling and dataloading starts to can take a significant percentage of the epoch time.

One notable exception is pubmed, in which case mini-batch training is slower than full graph training. This is because mini-batch training involves high graph sampling overhead, which occupies more than $90\%$ of the epoch time. Pubmed has such sampling overhead because of the fixed overhead in Minibatch sampling, which involves the shuffling of the root vertices at each epoch, making the sampling relatively expensive compared to the forward and backward costs. 

\begin{figure}[t]
    \includegraphics[width=\linewidth]{figures/mb_vs_full_cpu_4.pdf}
    \caption{Time to accuracy for GraphSage on a single CPU.}
    \label{fig:mb_vs_full_cpu}
\end{figure}

\input{tables/cpu_epoch_tta}

==> sections/22-memory-cost.tex <==
\begin{figure}[ht]
    \includegraphics[width=\linewidth]{figures/peak_mem_fg_mb_ratio.pdf}
    \caption{FG/MB ratio of per epoch peak memory for Pubmed, ogbn-arxiv, reddit, ogbn-products for GraphSAGE (single NVLink host). \ms{Is this Full-Graph vs. DGL + NS?}}
    \label{fig:peak_mem}
\end{figure}


==> tables/accuracy-convergence-graphsage-new.tex <==
\begin{table*}[t]
\caption{Accuracy (\%) of GraphSage using hyperparameter tuning method in Figure~\ref{fig:methodology}. \ms{Papers100M still incomplete.}}
\label{tab:convergence_graphsage}
    \begin{center}
    \begin{small}
    \tabcolsep=0.035cm
    % \vspace{-2pt}
    % \begin{sc}    
% \begin{tabular}{| m{3em} | m{3em} m{3em} | m{3em} m{3em}| m{3em} m{3em} |m{3em} m{3em} |m{3em} m{3em}|} 
\begin{tabular}{|l | l l | l l | l l  |l l |l l|} 
\toprule
 & \multicolumn{2}{c|}{Pubmed}  & \multicolumn{2}{c|}{Ogbn-arxiv} & \multicolumn{2}{c|}{Reddit} & \multicolumn{2}{c|}{Ogbn-products} & \multicolumn{2}{c|}{Ogbn-papers100M}\\
\midrule
%Metric & Training technique & \multicolumn{8}{c}{Architecure} \\
%\midrule
& FG-search & MB-search & FG-search & MB-search & FG-search & MB-search & FG-search & MB-search & FG-search & MB-search \\
\midrule
FG-train & $\textbf{77.40} \pm \textbf{00.04}$ & $76.10 \pm 00.67$ & $\textbf{71.76} \pm \textbf{00.16}$ & $67.21 \pm 00.9$ & $\textbf{96.94} \pm \textbf{00.01}$ & $90.28 \pm 00.63$ & $\textbf{79.29} \pm \textbf{00.15}$ & $76.60 \pm 00.32$ & $\textbf{62.82} \pm \textbf{00.01}$ & $61.74 \pm 00.13$ \\
MB-train & $77.00 \pm 00.39$ & $\textbf{84.03} \pm \textbf{00.61}$ & $70.73 \pm 00.38$ & $\textbf{73.80} \pm \textbf{00.13}$ & $96.52 \pm 00.14$ & $\textbf{98.40} \pm \textbf{00.03}$ & $78.72 \pm 00.07$ & $\textbf{79.50} \pm \textbf{00.17}$ & $62.52 \pm 00.04$  & $\textbf{62.77} \pm \textbf{00.02}$\\
% \midrule
% Epochs to converge & FG-train & 725 & 950 & 950 & 910 & 650 & 910 & 460 & 620 \\
% & MB-train & 175 & 170 & 135 & 210 & 120 & 100 & 235 & 165 \\
% \midrule
% Throughput (epochs/s) & PipeGCN &34.855 & 60.533 & 0.941 & 1.326 & 0.087& 0.152 & 0.088 & 0.076 \\
% & DGL & 28.783 & 37.281 & 0.337 & 0.304 & 0.068 & 0.120 & 0.074 & 0.052 \\
% \midrule
% Convergence time (s) & PipeGCN & 20.80 & 15.69 & 1009.08 & 686.14 & 7436.51 & 5985.73 & 5204.33 & 8157.90 \\
% & DGL & 6.08 & 4.56 & 400.74 & 691.610 & 1758.01 & 833.97 & 3182.24 & 3165.53 \\
      \bottomrule
\end{tabular}
    % \end{sc}
    \end{small}
    \end{center}
\end{table*}



==> tables/cpu_epoch_tta.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Time to accuracy and epoch time for GraphSage with single CPU host. \juelin{New table, merge this into Table 6?}}
\label{tab:cpu_epoch_tta}
\resizebox{0.85\columnwidth}{!}{%
\begin{tabular}{|c|cc|cccc|}
\hline
System & \multicolumn{2}{c|}{CPU Full} & \multicolumn{4}{c|}{CPU Mini-Batch} \\ \hline
Graph & \multicolumn{1}{c|}{ET (s)} & TTA (s) & \multicolumn{1}{c|}{Sample (s)} & \multicolumn{1}{c|}{F\&B (s)} & \multicolumn{1}{c|}{ET (s)} & TTA (s) \\ \hline
Pubmed & \multicolumn{1}{c|}{0.03} & \textbf{2.4} & \multicolumn{1}{c|}{0.56} & \multicolumn{1}{c|}{0.04} & \multicolumn{1}{c|}{0.6} & 14.9 \\ \hline
Arxiv & \multicolumn{1}{c|}{1.5} & 143 & \multicolumn{1}{c|}{2.0} & \multicolumn{1}{c|}{6.1} & \multicolumn{1}{c|}{8.1} & \textbf{121} \\ \hline
Reddit & \multicolumn{1}{c|}{22} & 2196 & \multicolumn{1}{c|}{8.6} & \multicolumn{1}{c|}{20.5} & \multicolumn{1}{c|}{29.1} & \textbf{379} \\ \hline
Product & \multicolumn{1}{c|}{53.9} & 5232 & \multicolumn{1}{c|}{13.4} & \multicolumn{1}{c|}{124.6} & \multicolumn{1}{c|}{138} & \textbf{3590} \\ \hline
\end{tabular}%
}
\end{table}

==> tables/time-to-acc-nvlink-multihost.tex <==
   
\begin{table}[t]
\caption{Time to accuracy and epoch time for GraphSage and ogbn-papers100M (3 NVLink hosts) }
\label{tab:time_to_acc_papers_nvlink}
    \begin{center}
    \begin{small}
    % \begin{sc}    
\begin{tabular}{| m{8em}| m{9em} |>{\raggedleft\arraybackslash}m{5em}|} 
\toprule
 & System & Time (s)\\
 % (\# Layers, Hidden size) & & (2,128)\\
\midrule
\multirow{3}{7em}{Epoch time (s)} 
& Full-Graph & 1.139 \\
& PipeGCN& \textbf{0.352} \\
& BNS-GCN&  0.432 \\
\cline{2-3}
& DistDGL &  4.452 \\
\midrule
\multirow{3}{7em}{Time to accuracy (s)} 
& Full-Graph &  1093.63 \\
& PipeGCN &  306.59 \\
& BNS-GCN&  133.92   \\
\cline{2-3}
& DistDGL& \textbf{ 35.62} \\
      \bottomrule
\end{tabular}
    % \end{sc}
    \end{small}
    \end{center}
\end{table}
